BlissCam: Boosting Eye Tracking Efficiency with Learned In-Sensor Sparse Sampling

Eye tracking is becoming an increasingly important task domain in emerging computing platforms such as Augmented/Virtual Reality (AR/VR). Today's eye tracking system suffers from long end-to-end tracking latency and can easily eat up half of the power budget of a mobile VR device. Most existing optimization efforts exclusively focus on the computation pipeline by optimizing the algorithm and/or designing dedicated accelerators while largely ignoring the front-end of any eye tracking pipeline: the image sensor. This paper makes a case for co-designing the imaging system with the computing system. In particular, we propose the notion of "in-sensor sparse sampling", whereby the pixels are drastically downsampled (by 20x) within the sensor. Such in-sensor sampling enhances the overall tracking efficiency by significantly reducing 1) the power consumption of the sensor readout chain and sensor-host communication interfaces, two major power contributors, and 2) the work done on the host, which receives and operates on far fewer pixels. With careful reuse of existing pixel circuitry, our proposed BLISSCAM requires little hardware augmentation to support the in-sensor operations. Our synthesis results show up to 8.2x energy reduction and 1.4x latency reduction over existing eye tracking pipelines.

==> ack.tex <==
\section{Acknowledgements}



==> coverpage.tex <==
\newpage

\noindent\textbf{\large $\bigstar$ Major Changes:}
\begin{itemize}
    \item We revised \Sect{sec:intro} to discuss the architectural contributions of the paper and why it is good for ISCA.
    The architecture contributions of our work are, in spirit, similar to the analog computing hardware (i.e. PIM hardware using crossbar, or in-memory computing) work published at ISCA before~\cite{shafiee2016isaac,guo2010resistive,li2020timely,imani2019floatpim,zou2022biohd}, and is in line with the ``Architectures for emerging technologies including novel circuits, memory technologies, quantum computing, etc.'' theme in the call for papers. (\underline{Reviewer A, B, E})
    \item We revised \Sect{sec:exp} (under ``Experimental Methodology'') to clarify how we obtain the results for 7 \si{\nano\meter} to 65 \si{\nano\meter} using the synthesis results from a 16 \si{\nano\meter} library. (\underline{Reviewer A})
    \item We revised \Sect{sec:eval:sen} (under ``Process Node'') to clearly describe how the technology node scaling is performed in sensitivity study. (\underline{Reviewer A})
    \item We revised \Sect{sec:eval:area} to include a component-level area breakdown and elaborate on our area estimation methodology, including why we do not estimate pixel area from pixel synthesis. (\underline{Reviewer A})
    \item We updated \Fig{fig:cis_energy_breakdown} with recent ADC papers to show that the trend (readout/ADC power is significant) still holds. (\underline{Reviewer A})
    \item We revised \Sect{sec:motiv:eye} (under ``Systems Specifications'') to explain why 120 Hz per eye tracking rate is necessary. (Reviewer B)
    \item We revised \Sect{sec:related} (under ``Computational Image Sensors'') to compare with RedEye. (\underline{Reviewer B})
    \item We added a new ``Event Cameras'' paragraph in \Sect{sec:related} to include a discussion of the motivation and the principle behind our eventification and ROI determination strategies.
    We are indeed inspired by event cameras but customize the design for eye tracking. (\underline{Reviewer B})
    \item We clarified in \Sect{sec:motiv:eye} that our eye tracking setup is for VR. (\underline{Reviewer C})
    \item We revised \Sect{sec:eval:acc} and \Fig{fig:acc} to include standard deviation of the accuracy data to show that our method is more robust against temporal eye dynamics like drift than the baselines. (\underline{Reviewer C})
    \item We added a new ``ROI Reuse'' paragraph in \Sect{sec:eval:sen} to show that reusing ROIs increases errors compared to using our ROI prediction network. (\underline{Reviewer C})
    \item We revised \Sect{sec:eval:perf} to include per-frame latency statistics/variations. (\underline{Reviewer C})

    \item We added a new ``Random Sampling Image Sensors'' paragraph in \Sect{sec:related} to discuss prior work on random sampling image sensors and highlight our contributions of random sampling with fine granularity and the ability to buffer the previous frame for eventification. (\underline{Reviewer D})
    \item We revised \Sect{sec:motiv:mot} (under ``Tracking Latency'') to explain the 15 \si{\milli\second} tracking latency. (\underline{Reviewer E})
\end{itemize}

\vspace{10pt}\noindent\textbf{\large $\bigstar$ Reviewer A}

\noindent\textbf{No optimization on in-sensor NPU.}

We have explicitly stated in the first paragraph of \Sect{sec:exp} that we do not claim any contributions to the NPU, and it is intentional: it shows that our sensor augmentation is compatible with a generic NPU and, thus, has wide applicability.


\noindent\textbf{The synthesis and verification results of the design (power, area, and timing) are missing.}

\Sect{sec:eval:area} has a component-level area breakdown.
\Fig{fig:energy} has a component-level power breakdown.
\Fig{fig:latency} has a component-level timing breakdown.

\vspace{10pt}\noindent\textbf{\large $\bigstar$ Reviewer B}

\noindent\textbf{Why does summing the 10 SRAM power-up bits mitigate the non-uniform randomness?
}

Based on the central limit theorem, as you pointed out.

\vspace{10pt}\noindent\textbf{\large $\bigstar$ Reviewer C}

\noindent\textbf{Need ablation studies to show how each of the algorithm components (eventification, ROI, segmentation) affects error, compression ratio, and latency/energy.}

Our three variants described in \Sect{sec:exp}-System Variants are meant for ablation studies.
More specifically, we perform three ablation studies.
First, we show that the accuracy using full frame (\mode{NPU-Full}) is only $0.41^{\circ}$ better but consumes $5.8\times$ more energy than our full pipeline.
Second, using ROI but without sampling (\mode{NPU-ROI}) increases the accuracy only by $0.09^{\circ}$ over our full pipeline but consumes 60\% more energy.
Both points above are shown in \Fig{fig:acc} and \Fig{fig:energy}.
Finally, \mode{S+NPU} runs sparse sampling in the digital and consumes 41\% more energy (same accuracy), showing the importance of in-pixel sampling (\Fig{fig:energy}).

%We revised \Sect{sec:exp}-System Variants to emphasize the setup of ablation studies.

\noindent\textbf{Were test images from OpenEDS, or a different one, used for the results in \Fig{fig:acc} to \Fig{fig:energy_profile}?}

We use the test images in OpenEDS.

\noindent\textbf{Do the test images vary across the experiments?}

No; they are all from OpenEDS and are used consistently throughout \Fig{fig:acc} to \Fig{fig:energy_profile}.

\vspace{10pt}\noindent\textbf{\large $\bigstar$ Reviewer D}

\noindent\textbf{Missing citations for the acceptable error thresholds.}

Please see \Sect{sec:motiv:eye}-System Specifications. We also mentioned those references again in \Sect{sec:eval:acc}.

\vspace{10pt}\noindent\textbf{\large $\bigstar$ Reviewer E}

\noindent\textbf{Missing background on basic in-sensor analog building blocks (ADC, etc.).}

The operation of the conventional ADC is described in the second paragraph in \Sect{sec:sensor:design}.

\noindent\textbf{Missing definition for ``MIPI''.}

We added the definition in \Sect{sec:motiv:cis}-Image Sensor Basics.

\noindent\textbf{How much of the total eye-tracking latency does the MIPI latency represent?}

The actual MIPI latency in a pipeline depends on the image resolution.  
Using the OpenEDS dataset, which has a resolution of $640\times400$, MIPI latency is about 10\% of the total latency (when ROI is used).
The MIPI latency will only increase as the image resolution increases, as shown in \Fig{fig:overview}.



==> overview.tex <==
\section{Overview}
\label{sec:oveview}

One key reason conventional DNNs are amenable to hardware acceleration is that their memory accesses are streaming and statically known. As a result, DRAM accesses can be overlapped with computation; SRAM accesses can be scheduled without stalling the Processing Element array. Point cloud networks exhibit irregular memory accesses. Building on top of the characterization results, the goal of the paper is to tame the irregular memory (DRAM and SRAM) accesses.

We first focus on DRAM. The main DRAM inefficiencies are introduced by neighbor search. We propose a new neighbor search algorithm that removes random DRAM accesses altogether and enable completely streaming DRAM traffic. As a byproduct, the algorithm also significantly reduces the DRAM traffic.

We then turn our attention to addressing the on-chip memory access inefficiencies. We show that SRAM accesses are input-dependent, leading to excessive bank conflicts that stall the datapath. Our idea is to elide bank conflicts at run time. While the hardware support for bank conflict elision is not complicated, it is not clear how to do so in a way that minimizes the accuracy impact.

The techniques above naturally sacrifice accuracy. Instead of empirically evaluate the accuracy, we aim for a systematic and principled approach to make accuracy-vs-performance trade-offs. In particular, our idea is to integrate the approximate operations into the network training process. In essence, by exposing the network to exactly how inference will be approximated, the network weights naturally learned to mitigate accuracy loss. Critically, we show that our network can make the trade-off in-situ at inference time without re-training.



==> system.tex <==
\section{System Design}
\label{sec:sys}

In this section, we first give an overview of our hardware architecture design (\Sect{sec:sys:arch}). Based on such architecture design, we discuss how to map our algorithm to the hardware and pipeline our algorithm (\Sect{sec:sys:pipeline}).

\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{arch_design}
    \caption{Overall architecture design}
    \label{fig:arch_design}
\end{figure}

\subsection{Hardware Architecture Design}
\label{sec:sys:arch}

\Fig{fig:arch_design} provides an overview of our architecture design, which includes two main components: a sparse sampling sensor and a DNN accelerator. The sparse sensing sampling sensor comprises a 3D stacked pixel array, an in-sensor MAC array, and an in-sensor buffer. The detailed description of the 3D stacked pixel array is already presented in \Sect{sec:sensor:design}. The in-sensor MAC array, on the other hand, consists of a systolic array-like PE array for convolution and a scalar unit to accelerate non-convolution operations such as ReLU. To ensure no extra data traffic off-sensor, the In-sensor buffer is employed to store temporary data, including intermediate feature maps and model weights of ROI prediction.

On the host SoC, there is a DNN accelerator to execute the sparse adaptive eye segmentation. Mirroring the architectural components within the sensor, this accelerator consists of a systolic array-like PE array and a scalar unit to accelerate non-convolution operations efficiently. Additionally, a global buffer is incorporated to hold model weights and intermediate results while communicating with DRAM. This global buffer is evenly split into two for double-buffering so that any data accessed by PEs would hit the buffer.

\subsection{Pipeline}
\label{sec:sys:pipeline}

To maximize the performance of our sparse sampled eye segmentation algorithm, we present our meticulously crafted pipeline laid out in \Fig{fig:pipeline}.

In our pipeline, at time $T_0$, each frame starts with the crucial step, exposure. As the frame approaches the end of the exposure, denoted as $T_1$ in \Fig{fig:pipeline}, we initiate the process of reading the voltage values from the pixel array while each pixel is continuing its exposure. These voltage values are used to generate an event map in the analog domain using the circuit described in \Sect{sec:sensor:design}. This event map is then written to the in-sensor buffer for ROI prediction. 

The in-sensor MAC array takes the event map and executes the ROI prediction network to generate the ROI result. This ROI result, in turn, is then used in the row and column decoder in the pixel array to set the row and column enable bits within each pixel. In the meantime, the SRAM within each pixel performs power-up to set the random sampling bit in each pixel. These three processes, row/column bit configuration and random sampling bit assignment, occur within the sparse sampling stage as illustrated in \Fig{fig:pipeline}. 
Eventification, ROI prediction, and sparse sampling are all performed concurrently with the pixel exposure to ensure that exposure time would not be affected by the extra in-sensor computing time. Three bits, row/column enable bit and random sampling bit, together determine whether to read out this given pixel via an three-operant AND operation. 

Following the pixel readout, selected pixel values are read out of the pixel array and dispatched to the host SoC via the MIPI CSI-2 interface. The host SoC receives the sparsely sampled pixels and executes the eye segmentation algorithm on these pixels to generate a segmentation map as described in \Sect{sec:algo:dnn}. This segmentation map is then used in edge detection to compute the edge map which is essential for ROI prediction. Once the edge map is produced, it would be sent back to the pixel sensor via the MIPI CSI-2 interface and signal the sensor to perform eventification for the next frame, $F_{t+1}$, while the host SoC performs the gaze prediction to compute the final gaze direction for the current frame $F_t$.

The temporal dynamics of our pipeline are punctuated by two critical timestamps as highlighted in \Fig{fig:pipeline}. The first timestamp, $T_0$, represents an important juncture during the exposure process. Extending the exposure time after eventification has two benefits: firstly, it ensures the integrity of the normal exposure, preventing the exposure time from being affected by the eventification. Secondly, early-terminated exposure would require an early reset for all pixels which is known to be power-intensive.

The second timestamp is $T_2$. In our pipeline, the next frame's ROI prediction hinges on receiving the edge map from the current frame. This dependency necessitates that the ROI prediction waits for the arrival of the edge map from the host SoC before executing it. These two critical timestamps, $T_0$ and $T_2$, are representations of the meticulous synchronization within our pipeline, underscoring the efficiency of our design.
